Application of Genetic Programming to High Energy Physics Event Selection

We review genetic programming principles, their application to FOCUS data samples, and use the method to study the doubly Cabibbo suppressed decay D+ -> K+ pi+ pi- relative to its Cabibbo favored counterpart, D+ -> K- pi+ pi+. We find that this technique is able to improve upon more traditional analysis methods. To our knowledge, this is the first application of the genetic programming technique to High Energy Physics data.

==> trees/dp_gen4_328.tex <==
\pstree{\gpop{$ \times $}}{\pstree{\gpop{max}}{\pstree{\gpop{$<$}}{\gpterm{Iso1}\gpterm{$\chi^2_{\pi1}$}}\pstree{\gpop{XOR}}{\pstree{\gpop{XOR}}{\gpterm{0.10}\gpterm{$\chi^2_{\pi2}$}}\pstree{\gpop{$<$}}{\gpterm{Clp}\gpterm{$\pi_{e2}$}}}}\pstree{\gpop{$ \times $}}{\pstree{\gpop{$ \times $}}{\gpterm{OoT}\gpterm{$\Delta \pion \kaon_1$}}\pstree{\gpop{XOR}}{\gpterm{POT}\gpterm{$\Sigma p^2_T$}}}}

